Influence and Passivity in Social Media

The ever-increasing amount of information flowing through Social Media forces the members of these networks to compete for attention and influence by relying on other people to spread their message. A large study of information propagation within Twitter reveals that the majority of users act as passive information consumers and do not forward the content to the network. Therefore, in order for individuals to become influential they must not only obtain attention and thus be popular, but also overcome user passivity. We propose an algorithm that determines the influence and passivity of users based on their information forwarding activity. An evaluation performed with a 2.5 million user dataset shows that our influence measure is a good predictor of URL clicks, outperforming several other measures that do not explicitly take user passivity into account. We also explicitly demonstrate that high popularity does not necessarily imply high influence and vice-versa.

==> input.tex <==
\section{The Input} \label{sec-input}
There are many ways of defining the influence graph $G=(N,E,W)$. We construct the
influence graph in 3 different ways taking into account URL mentions, retweets,
and the follower graph.

\subsection{The Mention/Follower Influence Graph}
The nodes of this graph are users who tweeted at least 3 URLs. The arc $(i,j)$
exists if user $j$ follows user $i$ and $j$ mentioned at least 1 URL that $i$ had
previously mentioned.  The arc $e=(i,j)$ has weight $w_e =
\frac{S_{ij}}{F_{ij}+S_{ij}}$ where $F_{ij}$ is the number of URLs that $i$
mentioned and $j$ never did and $S$ is the number of URLs mentioned by $j$ and
previously mentioned by $i$.

\subsection{The RT Influence Graph}
The nodes of this graph are users who tweeted at least 3 URLs. The arc $(i,j)$
exists if user $j$ retweeted a URL posted by user $i$ at least once.  The arc
$e=(i,j)$ has weight $w_e = \frac{S_{ij}}{P_{ij}}$ where $P_{i}$ is the number of
URLs that $i$ mentioned and $S_{ij}$ is the number of URLs mentioned by $i$ and
retweeted by $j$.

\subsection{The RT/Follower Influence Graph}
The nodes of this graph are users who tweeted at least 3 URLs. The arc $(i,j)$
exists if user $j$ follows user $i$ and user $j$ retweeted a URL posted by user
$i$ at least once.  The arc $e=(i,j)$ has weight $w_e = \frac{S_{ij}}{P_{ij}}$
where $P_{i}$ is the number of URLs that $i$ mentioned and $S_{ij}$ is the number
of URLs mentioned by $i$ and retweeted by $j$.

